Online structural health monitoring by model order reduction and deep learning algorithms

Within a structural health monitoring (SHM) framework, we propose a simulation-based classification strategy to move towards online damage localization. The procedure combines parametric Model Order Reduction (MOR) techniques and Fully Convolutional Networks (FCNs) to analyze raw vibration measurements recorded on the monitored structure. First, a dataset of possible structural responses under varying operational conditions is built through a physics-based model, allowing for a finite set of predefined damage scenarios. Then, the dataset is used for the offline training of the FCN. Because of the extremely large number of model evaluations required by the dataset construction, MOR techniques are employed to reduce the computational burden. The trained classifier is shown to be able to map unseen vibrational recordings, e.g. collected on-the-fly from sensors placed on the structure, to the actual damage state, thus providing information concerning the presence and also the location of damage. The proposed strategy has been validated by means of two case studies, concerning a 2D portal frame and a 3D portal frame railway bridge; MOR techniques have allowed us to respectively speed up the analyses about 30 and 420 times. For both the case studies, after training the classifier has attained an accuracy greater than 85%.

==> pgflibraryqrr.shapes.openrectangle.code.tex <==
\let\pgf@sh@openrectangle@full\pgf@sh@bg@rectangle
\let\pgf@sh@openrectangle@\pgf@sh@openrectangle@full
\def\pgf@sh@openrectangle@e    {\pgfsetrectcap\pgfpathmoveto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@n    {\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@w    {\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\NW}}
\def\pgf@sh@openrectangle@s    {\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@en{\pgfsetrectcap\pgfpathmoveto{\SE}\pgfpathlineto{\NE}\pgfpathlineto{\NW}}
\def\pgf@sh@openrectangle@ew{\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\SW}\pgfpathmoveto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@es{\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@enw{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\SE}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
  \pgfpathlineto{\NE}\pgfpathlineto{\NW}\pgfpathlineto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}}
\def\pgf@sh@openrectangle@ens{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}
  \pgfpathlineto{\SE}\pgfpathlineto{\NE}\pgfpathlineto{\pgfpointadd{\NW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}}
\def\pgf@sh@openrectangle@ews{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}
  \pgfpathlineto{\SE}\pgfpathlineto{\SW}\pgfpathlineto{\pgfpointadd{\NW}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
\def\pgf@sh@openrectangle@nw{\pgfsetrectcap\pgfpathmoveto{\NE}\pgfpathlineto{\NW}\pgfpathlineto{\SW}}
\def\pgf@sh@openrectangle@ns{\pgfsetrectcap\pgfpathmoveto{\NE}\pgfpathlineto{\NW}\pgfpathmoveto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@nws{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}
  \pgfpathlineto{\NW}\pgfpathlineto{\SW}\pgfpathlineto{\pgfpointadd{\SE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}
\def\pgf@sh@openrectangle@ws{\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@bbg@e{\pgfsetcornersarced{\pgfpointorigin}\pgfpathrectanglecorners{\southwest}{\northeast}}
\let\pgf@sh@openrectangle@bbg@n\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@s\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@w\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@ns\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@ew\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@full\pgf@sh@openrectangle@full
\let\pgf@sh@openrectangle@bbg@\pgf@sh@openrectangle@
\let\pgf@sh@openrectangle@bbg@enw\pgf@sh@openrectangle@enw
\let\pgf@sh@openrectangle@bbg@ens\pgf@sh@openrectangle@ens
\let\pgf@sh@openrectangle@bbg@ews\pgf@sh@openrectangle@ews
\let\pgf@sh@openrectangle@bbg@nws\pgf@sh@openrectangle@nws
\def\pgf@sh@openrectangle@bbg@en{%
  \pgfpathmoveto{\pgfpointadd{\SE}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
  \pgfpathlineto{\NE}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\NW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}%
  \pgfpathlineto{\southwest}}
\def\pgf@sh@openrectangle@bbg@nw{%
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}%
  \pgfpathlineto{\NW}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
  \pgfpathlineto{\southwest\pgf@ya\pgf@y\northeast\pgf@y\pgf@ya}}
\def\pgf@sh@openrectangle@bbg@ws{%
  \pgfpathmoveto{\pgfpointadd{\NW}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
  \pgfpathlineto{\SW}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\SE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}%
  \pgfpathlineto{\northeast}}
\def\pgf@sh@openrectangle@bbg@es{%
  \pgfpathmoveto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}%
  \pgfpathlineto{\SE}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\NE}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
  \pgfpathlineto{\southwest\pgf@xa\pgf@x\northeast\pgf@x\pgf@xa}}
\pgfset{open rectangle sides/.initial=ns, open rectangle fill/.initial=}
\pgfdeclareshape{open rectangle}{%
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}     \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{north west}\inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{north east}\inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}      \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{base}      \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{base west} \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{base east} \inheritanchor[from=rectangle]{mid east}
  \behindbackgroundpath{%
    \pgfkeysgetvalue{/pgf/open rectangle fill}\pgf@temp
    \ifx\pgf@temp\pgfutil@empty
    \else
      \pgfextract@process\SW{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
      \pgf@xa\pgf@x\pgf@ya\pgf@y
      \pgfextract@process\NE{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
      \pgf@xb\pgf@x\pgf@yb\pgf@y
      \pgfextract@process\NW{\pgf@x\pgf@xa\pgf@y\pgf@yb}%
      \pgfextract@process\SE{\pgf@x\pgf@xb\pgf@y\pgf@ya}%
      \csname pgf@sh@openrectangle@bbg@\pgfkeysvalueof{/pgf/open rectangle sides}\endcsname
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/open rectangle fill}}%
      \pgfusepath{fill}
    \fi
  }%
  \backgroundpath{%
    \pgfextract@process\SW{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
    \pgf@xa\pgf@x\pgf@ya\pgf@y
    \pgfextract@process\NE{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
    \pgf@xb\pgf@x\pgf@yb\pgf@y
    \pgfextract@process\NW{\pgf@x\pgf@xa\pgf@y\pgf@yb}%
    \pgfextract@process\SE{\pgf@x\pgf@xb\pgf@y\pgf@ya}%
    \csname pgf@sh@openrectangle@\pgfkeysvalueof{/pgf/open rectangle sides}\endcsname}}
\endinput


==> pgflibraryqrr.trans.code.tex <==
\def\pgftransformxmirror#1{
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared
    \pgf@xa\pgfmathresult pt\relax
    \advance\pgf@xa2\relax
    \pgftransformcm{-1}{0}{0}{1}{\pgfqpoint{+\the\pgf@xa}{+0pt}}%
  \else
    \pgftransformmirror{\pgfqpointxy{\pgfmathresult}{0}}{\pgfpointadd{\pgfqpointxy{\pgfmathresult}{0}}{\pgfqpointxy{0}{1}}}%
  \fi
}
\def\pgftransformymirror#1{
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared
    \pgf@ya\pgfmathresult pt\relax
    \advance\pgf@ya2\relax
    \pgftransformcm{1}{0}{0}{-1}{\pgfqpoint{+0pt}{+\the\pgf@ya}}%
  \else
    \edef\pgf@marshal{\noexpand\pgftransformmirror{\noexpand\pgfqpointxy{0}{\pgfmathresult}}%
                                                  {\noexpand\pgfpointadd{\noexpand\pgfqpointxy{0}{\pgfmathresult}}{\noexpand\pgfqpointxy{1}{0}}}}%
    \pgf@marshal
  \fi}
\def\pgftransformmirror#1#2{%
  \pgfextract@process\pgf@tempa{#1}%
  \pgfpointnormalised{\pgfpointdiff{\pgf@tempa}{#2}}%
  \pgf@xa=\pgf@sys@tonumber\pgf@y\pgf@x
  \pgf@xb=\pgf@sys@tonumber\pgf@x\pgf@x
  \pgf@yb=\pgf@sys@tonumber\pgf@y\pgf@y
  \multiply\pgf@xa2\relax
  \pgf@xc=-\pgf@yb\advance\pgf@xc\pgf@xb
  \pgf@yc=-\pgf@xb\advance\pgf@yc\pgf@yb
  \edef\pgf@temp{{\the\pgf@xc}{+\the\pgf@xa}{+\the\pgf@xa}{+\the\pgf@yc}}%
  \expandafter\pgf@transformcm\pgf@temp{\pgf@tempa}%
  \pgftransformshift{\pgfpointscale{-1}{\pgf@tempa}}%
}
\def\pgfqtransformmirror#1{%
  \pgfpointnormalised{#1}%
  \pgf@xa=\pgf@sys@tonumber\pgf@y\pgf@x
  \pgf@xb=\pgf@sys@tonumber\pgf@x\pgf@x
  \pgf@yb=\pgf@sys@tonumber\pgf@y\pgf@y
  \multiply\pgf@xa2\relax
  \pgf@xc=-\pgf@yb\advance\pgf@xc\pgf@xb
  \pgf@yc=-\pgf@xb\advance\pgf@yc\pgf@yb
  \edef\pgf@temp{{\the\pgf@xc}{+\the\pgf@xa}{+\the\pgf@xa}{+\the\pgf@yc}}%
  \expandafter\pgf@transformcm\pgf@temp{\pgfpointorigin}%
}
\endinput


==> pgflibraryshapes.qrr.roundedrectangle.code.tex <==
\input tikzlibraryshapes.qrr.roundedrectangle.code.tex
\endinput


==> tikzlibrarynode-families.code.tex <==
\let\tikz@lib@nf@textheight\relax
\let\tikz@lib@nf@textdepth\relax
\let\tikz@lib@nf@textwidth\relax
\tikzset{
  Minimum Width/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@width}{}{%
      \tikzset{/tikz/minimum width/.expand twice=+\csname\pgfpictureid @#1@width\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}\global\let\tikz@lib@nf@outerxsep\tikz@lib@nf@outerxsep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{east}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{west}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \pgfutil@ifundefined{\pgfpictureid @#1@width}{%
              \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@width\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{width}{width}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Height/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@height}{}{%
      \tikzset{/tikz/minimum height/.expand twice=+\csname\pgfpictureid @#1@height\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerysep{\pgfkeysvalueof{/pgf/outer ysep}}\global\let\tikz@lib@nf@outerysep\tikz@lib@nf@outerysep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{north}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{south}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \pgfutil@ifundefined{\pgfpictureid @#1@height}{%
              \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@height\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{height}{height}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Size/.style={
    Minimum Height={#1},
    Minimum Width={#1}},
  Text Height/.code=\edef\tikz@lib@nf@textheight{#1},
  Text Depth/.code= \edef\tikz@lib@nf@textdepth{#1},
  Text Width/.code=%
    \edef\tikz@lib@nf@textwidth{#1}%
    \pgfutil@ifundefined{\pgfpictureid @#1@textwidth}{}{%
      \tikzset{text width/.expand twice=+\csname\pgfpictureid @#1@textwidth\endcsname}%
    }%
}

\def\tikz@lib@nf@text@#1#2#3{%
  \expandafter\ifx\csname tikz@lib@nf@#3\endcsname\relax\else
    \ifx#1\wd\def\tikz@temp{@}\else\let\tikz@temp\pgfutil@empty\fi
    \expandafter\ifx\csname tikz@lib@nf@#3\tikz@temp\endcsname\pgfutil@empty\else
      \pgfutil@ifundefined{\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp}{%
        \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
      }{%
        \ifdim\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname<#1#2
          \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
        \else
          \ifx#1\wd\else
            #1#2=\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\endcsname\relax
          \fi
        \fi
      }%
      \edef\tikz@temp{\noexpand\tikz@lib@nf@save{\pgfpictureid}{\csname tikz@lib@nf@#3\endcsname}{#3}{#3\tikz@temp}}%
      \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
      \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\tikz@temp}%
    \fi
  \fi
}
%%% Redefinition
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    %
    %
    \tikz@lib@nf@text@\ht\pgfnodeparttextbox{textheight}%
    \tikz@lib@nf@text@\dp\pgfnodeparttextbox{textdepth}%
    \tikz@lib@nf@text@\wd\pgfnodeparttextbox{textwidth}%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}
\def\tikz@lib@nf@save#1#2#3#4{%
  \pgfutil@ifundefined{#1@#2@#3@done}{%
    \expandafter\let\csname#1@#2@#3@done\endcsname\pgfutil@empty%
    \immediate\write\pgfutil@auxout{\noexpand\expandafter\noexpand\gdef\noexpand\csname#1@#2@#3\endcsname{\csname#1@#2@#4\endcsname}}
  }{}%
}
\endinput


==> tikzlibrarynorm.code.tex <==
\tikzset{
	Norm/.code={%
		\pgfmathparse{#1}%
		\edef\qrr@tikz@norm{\pgfmathresult\ifpgfmathunitsdeclared pt\fi}%
		\let\ifqrr@tikz@normcs@unitsdeclared\ifpgfmathunitsdeclared},
	Norm=1,
	norm/.style={to path={-- ++(norm cs: \tikztotarget\space from \tikztostart) \tikztonodes}}
}
\newif\ifqrr@tikz@normcs@unitsdeclared
\newdimen\qrr@pgf@normcs@from@x\newdimen\qrr@pgf@normcs@from@y
\tikzdeclarecoordinatesystem{norm}{%
	\begingroup
		\let\qrr@next\relax
		\pgfutil@in@{ for }{#1}%
		\ifpgfutil@in@
			\qrr@tikz@normcs@parse@for#1\@qrr@tikz@normcs@parse@for
		\else
			\def\pgf@tempa{#1}%
		\fi
		\edef\pgf@marshal{\noexpand\pgfutil@in@{ from }{\pgf@tempa}}\pgf@marshal
		\ifpgfutil@in@
			\expandafter\qrr@tikz@normcs@parse@from\pgf@tempa\@qrr@tikz@normcs@parse@from
			\let\qrr@next\qrr@tikz@normcs@calc@hard
		\else
			\let\qrr@tikz@normcs@parse@to\pgf@tempa
			\qrr@pgf@normcs@from@x\z@
			\qrr@pgf@normcs@from@y\z@
		\fi
		\expandafter\qrr@tikz@normcs@parse@@to\expandafter{\qrr@tikz@normcs@parse@to}%
}
\def\qrr@tikz@normcs@calc@easy#1{%
	\pgf@xx\@ne
	\pgf@yy\@ne
	\pgf@xy\z@
	\pgf@yx\z@
	\tikz@scan@one@point\pgfutil@firstofone(#1)\relax
	\pgf@xa\pgf@x\pgf@ya\pgf@y
}
\def\qrr@tikz@normcs@calc@hard#1{%
	\tikz@scan@one@point\pgfutil@firstofone(#1)\relax
	\pgf@xa\pgf@x\pgf@ya\pgf@y
	\advance\pgf@xa-\qrr@pgf@normcs@from@x
	\advance\pgf@ya-\qrr@pgf@normcs@from@y
	\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}
	\pgfmathsetlength\pgf@xa{\pgf@yy*\pgf@x-\pgf@yx*\pgf@y}
	\pgfmathsetlength\pgf@ya{-\pgf@xy*\pgf@x+\pgf@xx*\pgf@y}
}
\def\qrr@tikz@normcs@calc@unit#1{%
	\tikz@scan@one@point\pgfutil@firstofone(#1)\relax
	\pgf@xa\pgf@x\pgf@ya\pgf@y
	\advance\pgf@xa-\qrr@pgf@normcs@from@x
	\advance\pgf@ya-\qrr@pgf@normcs@from@y
	\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}
	\pgf@xa\pgf@x\pgf@ya\pgf@y
}
\def\qrr@tikz@normcs@parse@@to#1{%
		\ifqrr@tikz@normcs@unitsdeclared
			\let\qrr@next\qrr@tikz@normcs@calc@unit
		\else
			\ifx\qrr@next\relax
			  \pgfutil@in@{cs:}{#1}%
			  \ifpgfutil@in@
			    \let\qrr@next\qrr@tikz@normcs@calc@hard
			  \else
			    \pgfutil@in@{intersection }{#1}%
			    \ifpgfutil@in@
			      \let\qrr@next\qrr@tikz@normcs@calc@hard
			    \else
			      \pgfutil@in@|{#1}%
			      \ifpgfutil@in@
			        \let\qrr@next\qrr@tikz@normcs@calc@hard
			      \else
			        \pgfutil@in@:{#1}%
			        \ifpgfutil@in@
			          \let\qrr@next\qrr@tikz@normcs@calc@easy
			        \else
			          \pgfutil@in@,{#1}%
			          \ifpgfutil@in@
			            \let\qrr@next\qrr@tikz@normcs@calc@easy
			          \else
			            \let\qrr@next\qrr@tikz@normcs@calc@hard
			          \fi
			        \fi
			      \fi
			    \fi
			  \fi
			\fi
		\fi
		\qrr@next{#1}%
		\pgfmathatantwo{+\pgf@xa}{+\pgf@ya}%
		\ifqrr@tikz@normcs@unitsdeclared
			\edef\pgf@marshal{\noexpand\pgfpointpolar{\pgfmathresult}{\qrr@tikz@norm}}
		\else
			\edef\pgf@marshal{\noexpand\pgfpointpolarxy{\pgfmathresult}{\qrr@tikz@norm}}
		\fi
		\pgfmath@smuggleone\pgf@marshal
	\endgroup
	\pgf@marshal

}

\def\qrr@tikz@normcs@parse@from#1 from #2\@qrr@tikz@normcs@parse@from{%
	\def\qrr@tikz@normcs@parse@to{#1}%
	\tikz@scan@one@point\pgfutil@firstofone(#2)\relax
	\qrr@pgf@normcs@from@x\pgf@x
	\qrr@pgf@normcs@from@y\pgf@y
}
\def\qrr@tikz@normcs@parse@for#1 for #2\@qrr@tikz@normcs@parse@for{%
	\def\pgf@tempa{#1}%
	\pgfkeysalso{/tikz/Norm={#2}}%
}

% a fix for the 2.10 version of PGF/TikZ
\expandafter\let\expandafter\pgfmathatantwo\csname pgfmathatan2\endcsname


==> tikzlibrarypaths.ortho.code.tex <==
\let\tikz@orig@rect\tikz@rect
\def\tikz@rect{\pgfutil@ifnextchar e\tikz@orig@rect\qrr@tikz@r}
\def\qrr@tikz@r -{%
  \pgfutil@ifnextchar l\qrr@tikz@lr@lineto{%
    \pgfutil@ifnextchar r\qrr@tikz@rl@lineto{%
      \pgfutil@ifnextchar u\qrr@tikz@ud@lineto{%
        \pgfutil@ifnextchar d\qrr@tikz@du@lineto\tikz@expand
      }%
    }%
  }%
}
\let\tikz@orig@vh@lineto@next\tikz@vh@lineto@next
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar|{\expandafter\qrr@tikz@vhv@lineto\pgfutil@gobble}%
    {\pgfutil@ifnextchar\tikz@activebar{\expandafter\qrr@tikz@vhv@lineto\pgfutil@gobble}%
      {\tikz@orig@vh@lineto@next}}}
\let\tikz@orig@hv@lineto\tikz@hv@lineto
\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar-{\expandafter\qrr@tikz@hvh@lineto\pgfutil@gobble}%
    {\tikz@orig@hv@lineto}}
\tikzset{%
  |-|/.style={%
   /utils/exec=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},%
   to path={|-| (\tikztotarget) \tikztonodes}},%
  -|-/.style={%
   /utils/exec=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},%
   to path={-|- (\tikztotarget) \tikztonodes}},%
  ud/.style={%
    udlr/ud distance/.expanded={#1},%
    to path={r-ud (\tikztotarget) \tikztonodes}},%
  du/.style={%
    udlr/du distance/.expanded={#1},%
    to path={r-du (\tikztotarget) \tikztonodes}},%
  lr/.style={%
    udlr/lr distance/.expanded={#1},%
    to path={r-lr (\tikztotarget) \tikztonodes}},%
  rl/.style={%
    udlr/rl distance/.expanded={#1},%
    to path={r-rl (\tikztotarget) \tikztonodes}},%
  ud/.default=\pgfkeysvalueof{/tikz/udlr/ud distance},%
  du/.default=\pgfkeysvalueof{/tikz/udlr/du distance},%
  rl/.default=\pgfkeysvalueof{/tikz/udlr/rl distance},%
  lr/.default=\pgfkeysvalueof{/tikz/udlr/lr distance},%
  |-|/.default=\qrr@tikz@hvvh@ratio,%
  -|-/.default=\qrr@tikz@hvvh@ratio
}

%BEGIN_FOLD hvvh operator
\def\qrr@tikz@vhv@lineto{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@vhv@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@vhv@lineto@next[]}}
\def\qrr@tikz@hvh@lineto{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@hvh@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@hvh@lineto@next[]}}
%END_FOLD

%BEGIN_FOLD udlr operators
%% ud style
\def\qrr@tikz@rl@lineto rl{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@rl@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@rl@lineto@next[]}}
\def\qrr@tikz@lr@lineto lr{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@lr@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@lr@lineto@next[]}}
\def\qrr@tikz@du@lineto du{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@du@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@du@lineto@next[]}}
\def\qrr@tikz@ud@lineto ud{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@ud@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@ud@lineto@next[]}}
%END_FOLD

\input tikzlibrarypaths.ortho.tex
\endinput


==> tikzlibrarypaths.ortho.tex <==
\newlength\qrr@tikz@udlr@distance
\newlength\qrr@tikz@hvvh@distance
\newif\ifqrr@tikz@hvvh@middle
\newif\ifqrr@tikz@hvvh@fromcenter
\newif\iftikz@ortho@preflush
\tikz@ortho@preflushtrue
\let\tikz@origtotarget\pgfutil@empty

%%% |-/-|
\tikzset{
  |-/.style={to path={|- (\tikztotarget) \tikztonodes}},
  -|/.style={to path={-| (\tikztotarget) \tikztonodes}},
  *|/.style={to path={%
    \pgfextra
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztostart{\tikztostart.north}%
        \else
          \edef\tikztostart{\tikztostart.south}%
        \fi
      \fi
    \endpgfextra
    (perpendicular cs: horizontal line through={(\tikztostart)},
                       vertical line through={(\tikztotarget)}) -- (\tikztotarget) \tikztonodes
  }},
  *-/.style={to path={%
    \pgfextra
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztostart{\tikztostart.east}%
        \else
          \edef\tikztostart{\tikztostart.west}%
        \fi
      \fi
    \endpgfextra
    (perpendicular cs: vertical line through={(\tikztostart)},
                     horizontal line through={(\tikztotarget)}) -- (\tikztotarget) \tikztonodes
  }},
  |*/.style={to path={%
    \pgfextra
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \iftikz@shapeborder
        \let\tikz@origtotarget\tikztotarget
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztotarget{\tikztotarget.south}%
        \else
          \edef\tikztotarget{\tikztotarget.north}%
        \fi
      \fi
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: vertical line through={(\tikztostart)},
                                         horizontal line through={(\tikztotarget)})
    \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
  }},
  -*/.style={to path={%
    \pgfextra
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \iftikz@shapeborder
        \let\tikz@origtotarget\tikztotarget
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztotarget{\tikztotarget.west}%
        \else
          \edef\tikztotarget{\tikztotarget.east}%
        \fi
      \fi
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: horizontal line through={(\tikztostart)},
                                         vertical line through={(\tikztotarget)})
    \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
  }},
  node as new start/.is if=tikz@ortho@preflush
}

%%% HVVH/UDLR
\tikzset{
  hvvh/.code={\pgfqkeys{/tikz/hvvh}{#1}},%
  udlr/.code={\pgfqkeys{/tikz/udlr}{#1}},%
%  hvvh/.search also=/tikz/udlr,%
  udlr/.search also=/tikz/hvvh,% endless loop?
  hvvh/middle 0 to 1/.style={hvvh/spacing=0},%
  hvvh/0 to 1/.style={hvvh/middle 0 to 1},%
  hvvh/from center/.is if=qrr@tikz@hvvh@fromcenter,%
  udlr/from center/.style={/tikz/hvvh/from center={#1}},
  udlr/from center/.default=true,
  hvvh/spacing/.code=%
    \ifcase#1\relax
      \qrr@tikz@hvvh@middletrue
      \def\qrr@tikz@hvvh@timing@parts{1}%
      \def\qrr@tikz@hvvh@timing@first{0}%
      \def\qrr@tikz@hvvh@timing@last{1}%
      \def\qrr@tikz@hvvh@timing@subtr{0}%
      \def\qrr@tikz@hvvh@timing@factor{1}%
    \else
      \qrr@tikz@hvvh@middlefalse
      \def\qrr@tikz@hvvh@timing@parts{#1}%
      \pgfmathreciprocal{#1}\let\qrr@tikz@hvvh@timing@first\pgfmathresult
      \pgfmathsetmacro\qrr@tikz@hvvh@timing@last{1-\pgfmathresult}%
      \pgfmathreciprocal{#1-2}%
      \let\qrr@tikz@hvvh@timing@subtr\pgfmathresult
      \pgfmathsetmacro\qrr@tikz@hvvh@timing@factor{1+2*\pgfmathresult}%
    \fi,
  hvvh/ratio/.code=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},
  hvvh/distance/.code=\pgfmathsetlength\qrr@tikz@hvvh@distance{#1}\let\qrr@tikz@hvvh@ratio\pgfutil@empty,%
  udlr/distance/.style={/tikz/udlr/ud distance={#1},/tikz/udlr/du distance={#1},/tikz/udlr/lr distance={#1},/tikz/udlr/rl distance={#1}},%
  udlr/ud distance/.initial=+.5cm,%
  udlr/du distance/.initial=+.5cm,%
  udlr/lr distance/.initial=+.5cm,%
  udlr/rl distance/.initial=+.5cm%
}
\tikzset{% default
  hvvh/ratio=.5,%
  hvvh/spacing=4%
}

%BEGIN_FOLD Timer
\def\tikz@timer@hvhline{%
  \pgf@process{\tikz@timer@start}\pgf@ya\pgf@y
  \pgf@process{\tikz@timer@end}\pgf@yc\pgf@y
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\qrr@tikz@hvvh@timing@first pt% first quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
  \else
    \ifdim\tikz@time pt>\qrr@tikz@hvvh@timing@last pt% last quarter
      \ifqrr@tikz@hvvh@middle
        \advance\pgf@xb-1pt%
      \else
        \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
      \fi
      \advance\pgf@xb\dimexpr-\qrr@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@yc}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb\qrr@tikz@hvvh@timing@factor\pgf@xb%
      \advance\pgf@xb-\qrr@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@middle}}%
    \fi\fi\tikz@marshal}
\def\tikz@timer@vhvline{%
  \pgf@process{\tikz@timer@start}\pgf@xa\pgf@x
  \pgf@process{\tikz@timer@end}\pgf@xc\pgf@x
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\qrr@tikz@hvvh@timing@first pt% first quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
  \else
    \ifdim\tikz@time pt>\qrr@tikz@hvvh@timing@last pt% last quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb-1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
      \advance\pgf@xb by\dimexpr-\qrr@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb=\qrr@tikz@hvvh@timing@factor\pgf@xb
      \advance\pgf@xb by-\qrr@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@middle}}%
      \fi\fi\tikz@marshal}

%END_FOLD
\let\tikz@hvvh@currentoption\pgfutil@empty
\def\qrr@tikz@collect@hvvh@options#1[#2]{\edef\tikz@hvvh@currentoption{#2}#1}
\def\qrr@tikz@hvh@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@hvh@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@hvh@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@hvh@lineto@next}{\tikz@scan@one@point\qrr@tikz@@hvh@lineto}}}}
\def\qrr@tikz@vhv@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@vhv@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@vhv@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@vhv@lineto@next}{\tikz@scan@one@point\qrr@tikz@@vhv@lineto}}}}
\def\qrr@tikz@ud@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@ud@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@ud@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@ud@lineto@next}{\tikz@scan@one@point\qrr@tikz@@ud@lineto}}}}
\def\qrr@tikz@du@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@du@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@du@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@du@lineto@next}{\tikz@scan@one@point\qrr@tikz@@du@lineto}}}}
\def\qrr@tikz@lr@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@lr@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@lr@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@lr@lineto@next}{\tikz@scan@one@point\qrr@tikz@@lr@lineto}}}}
\def\qrr@tikz@rl@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@rl@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@rl@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@rl@lineto@next}{\tikz@scan@one@point\qrr@tikz@@rl@lineto}}}}

\def\tikz@do@hvvh#1#2#3#4#5{%
% #1 = first kink
% #2 = second kink
% #3 = end
% #4 = timer
% #5 = tikz@shapeborder@name
  \pgfpathlineto{#1}%
  \pgfpathlineto{#2}%
  \pgfpathlineto{#3}%
  \def\tikz@timer@middle{#2}%
  \def\tikz@timer@end{#3}%
  \let\tikz@timer#4
  \edef\pgf@temp{#5}%
  \ifx\pgf@temp\pgfutil@empty
    \let\tikz@moveto@waiting\relax
  \else
    \edef\tikz@moveto@waiting{#5}%
  \fi
  \tikz@scan@next@command%
}
%BEGIN_FOLD hvvh operator
%% -|- operator
\def\qrr@tikz@@hvh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb=\tikz@lastx
  \pgf@xc=\tikz@lastx
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/hvvh}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xb}{\tikz@lasty}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \ifqrr@tikz@hvvh@fromcenter
            \pgf@xc\tikz@lastx
          \else
            \pgf@xc\pgf@x
          \fi
        \fi
        \ifdim\pgf@x>\tikz@lastx
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \ifqrr@tikz@hvvh@fromcenter
          \qrr@tikz@hvvh@distance\tikz@lastx
        \else
          \qrr@tikz@hvvh@distance\pgf@x
        \fi
        \advance\qrr@tikz@hvvh@distance-\pgf@xc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@xc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \pgf@xc\tikz@lastx
        \fi
        \ifdim\pgf@x>\tikz@lastx
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \qrr@tikz@hvvh@distance\tikz@lastx
        \advance\qrr@tikz@hvvh@distance-\pgf@xc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@xc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% |-| operator
\def\qrr@tikz@@vhv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx
  \pgf@yb=\tikz@lasty
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/hvvh}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yb}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \ifqrr@tikz@hvvh@fromcenter
            \pgf@yc\tikz@lasty
          \else
            \pgf@yc\pgf@y
          \fi
        \fi
        \ifdim\pgf@y>\tikz@lasty
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \ifqrr@tikz@hvvh@fromcenter
          \qrr@tikz@hvvh@distance\tikz@lasty
        \else
          \qrr@tikz@hvvh@distance\pgf@y
        \fi
        \advance\qrr@tikz@hvvh@distance-\pgf@yc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \pgf@yc\tikz@lasty
        \fi
        \ifdim\pgf@y>\tikz@lasty
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \qrr@tikz@hvvh@distance\tikz@lasty
        \advance\qrr@tikz@hvvh@distance-\pgf@yc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% ud operator
\def\qrr@tikz@@ud@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/ud distance}}%
    \iftikz@shapeborder
      \advance\pgf@y1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc<\pgf@y
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb<\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb\qrr@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% du operator
\def\qrr@tikz@@du@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/du distance}}%
    \iftikz@shapeborder
      \advance\pgf@y-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc>\pgf@y
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc-\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb>\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb-\qrr@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% lr operator
\def\qrr@tikz@@lr@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/lr distance}}%
    \iftikz@shapeborder
      \advance\pgf@x-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc>\pgf@x
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc-\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb>\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb-\qrr@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% rl operator
\def\qrr@tikz@@rl@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/rl distance}}%
    \iftikz@shapeborder%
      \advance\pgf@x1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc<\pgf@x
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty%
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb<\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb\qrr@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}
%END_FOLD
\endinput


==> tikzlibrarypaths.rectangle.code.tex <==
% This is the TikZ library paths.rectangle
% Load with \usetikzlibrary{paths.rectangle}
%
% This small library extends the node placing algorithm (a.k.a. timer)
% so that nodes can be placed on the path of an rectangle.
%
% Styles are:
%  - rectangle original timer
%    The original placement between position 0 and 1 are not changed.
%    The rectangle's path can be accessed by positions between 1 and 2.
%  - rectangle new timer
%    This style switches the positions between 0 and 1 with those
%    between 1 and 2.

\def\qrr@tikz@timer@rect@origline{%
  \ifdim\tikz@time pt>1pt
    \pgfutil@tempdima\tikz@time pt
    \ifdim\pgfutil@tempdima<1.5pt
      \advance\pgfutil@tempdima-1pt
    \else
      \advance\pgfutil@tempdima-1.5pt
      \let\pgf@tempa\tikz@timer@start
      \let\tikz@timer@start\tikz@timer@end
      \let\tikz@timer@end\pgf@tempa
    \fi
    \multiply\pgfutil@tempdima2
    \edef\tikz@time{\strip@pt\pgfutil@tempdima}%
    \expandafter\tikz@timer@vhline
  \else\expandafter\tikz@timer@line\fi
}
\def\qrr@tikz@timer@rect@lineafterone{%
  \pgfutil@tempdima\tikz@time pt
  \ifdim\pgfutil@tempdima<1pt
    \ifdim\pgfutil@tempdima<.5pt\else
      \advance\pgfutil@tempdima-.5pt
      \let\pgf@tempa\tikz@timer@start
      \let\tikz@timer@start\tikz@timer@end
      \let\tikz@timer@end\pgf@tempa
    \fi
    \multiply\pgfutil@tempdima2
    \edef\tikz@time{\strip@pt\pgfutil@tempdima}%
    \expandafter\tikz@timer@vhline
  \else
    \advance\pgfutil@tempdima-1pt
    \edef\tikz@time{\strip@pt\pgfutil@tempdima}%
    \expandafter\tikz@timer@line
  \fi
}
\tikzset{
  rectangle original timer/.code=\let\tikz@timer@line\qrr@tikz@timer@rect@origline,
  rectangle new timer/.code=\let\tikz@timer@line\qrr@tikz@timer@rect@lineafterone,
  rectangle original timer
}


==> tikzlibrarypatterns.images.code.tex <==
% This is the TikZ library patterns.images
% Load with \usetikzlibrary{patterns.images}
%
% Macro:
%  - \pgfSetupImageAsPattern[<opt arguments for \pgfdeclareimage>]{<name>}{<path/file>}
%
% Keys are:
%  - use image as pattern=<name>
%  - image as pattern=<opt arguments for \pgftext>

\newlength\qrr@pgf@iap@width
\newlength\qrr@pgf@iap@height

\def\pgfSetupImageAsPattern{\pgfutil@ifnextchar[\qrr@pgfSetupImageAsPattern{\qrr@pgfSetupImageAsPattern[]}}
\def\qrr@pgfSetupImageAsPattern[#1]#2#3{% #1 = options
                                        % #2 = image name
                                        % #3 = file name
  \pgfdeclareimage[#1]{qrr@pgf@iap@#2}{#3}%
  \sbox\pgfutil@tempboxa{\pgfuseimage{qrr@pgf@iap@#2}}%
  \expandafter\edef\csname qrr@pgf@iap@#2@width\endcsname{\the\wd\pgfutil@tempboxa}%
  \expandafter\edef\csname qrr@pgf@iap@#2@height\endcsname{\the\ht\pgfutil@tempboxa}%
}
\tikzset{
  image as pattern/.code={
    \edef\qrr@pgf@iap@options{#1}%
    \pgfkeysalso{/tikz/path picture={%
      \pgf@process{\pgfpointanchor{path picture bounding box}{north east}}%
      \pgf@xa\pgf@x\pgf@ya\pgf@y
      \pgf@process{\pgfpointanchor{path picture bounding box}{south west}}%
      \pgf@xb\pgf@x\pgf@yb\pgf@y\pgf@yc\pgf@yb
      \pgfutil@loop
        {%
        \pgfutil@loop
          \expandafter\pgftext\expandafter[\qrr@pgf@iap@options,at=\pgfqpoint{\pgf@xb}{\pgf@yb}]{\pgfuseimage{qrr@pgf@iap@\qrr@pgf@iap@name}}%
          \ifdim\pgf@yb<\pgf@ya
          \advance\pgf@yb\qrr@pgf@iap@height
        \pgfutil@repeat
        }%
        \ifdim\pgf@xb<\pgf@xa
        \advance\pgf@xb\qrr@pgf@iap@width
        \pgf@yb\pgf@yc
      \pgfutil@repeat
    }}%
  },
  use image as pattern/.code={%
    \edef\qrr@pgf@iap@name{#1}%
    \expandafter\qrr@pgf@iap@width\csname qrr@pgf@iap@#1@width\endcsname
    \expandafter\qrr@pgf@iap@height\csname qrr@pgf@iap@#1@height\endcsname
  }
}
\endinput


==> tikzlibrarypositioning-plus.code.tex <==
% This is the TikZ library positioning-plus
% Load with \usetikzlibrary{positioning-plus}
%
% This small library extends TikZ options like 'above', 'left' or 'below right'
% so that they can be used with an optional prefixed factor seperated by ':' (colon)
%
% The option 'left=.5:of somenode' will place
% a new node .5cm (default 'node distance' is '1cm and 1cm') left to (somenode).
% The option 'above right=.2 and .7:of someothernode' will place
% a new node .2cm above and .7cm right of (someothernode).
%
% Additional the options 'xshift*' and 'yshift*' add an additional shift
% as a factor of 'node distance'
% Inspired by http://tex.stackexchange.com/a/117610/16595

\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\pgfdeclaregenericanchor{corner south east}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north east}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner south west}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north west}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}

\tikzset{corner above left/.code=\tikz@lib@place@handle@{#1}{corner south east}{-1}{1}{corner north west}{0.707106781}}
\tikzset{corner above right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{1}{corner north east}{0.707106781}}
\tikzset{corner below left/.code=\tikz@lib@place@handle@{#1}{corner north east}{-1}{-1}{corner south west}{0.707106781}}
\tikzset{corner below right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{-1}{corner south east}{0.707106781}}

\tikzset{corner north left/.code =\tikz@lib@place@handle@{#1}{corner north east}{-1}{0}{corner north west}{1}}
\tikzset{corner north right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{0}{corner north east}{1}}
\tikzset{corner south left/.code =\tikz@lib@place@handle@{#1}{corner south east}{-1}{0}{corner south west}{1}}
\tikzset{corner south right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{0}{corner south east}{1}}

\tikzset{corner west above/.code =\tikz@lib@place@handle@{#1}{corner south west}{0}{1}{corner north west}{1}}
\tikzset{corner west below/.code=\tikz@lib@place@handle@{#1}{corner north west}{0}{-1}{corner south west}{1}}
\tikzset{corner east above/.code =\tikz@lib@place@handle@{#1}{corner south east}{0}{1}{corner north east}{1}}
\tikzset{corner east below/.code=\tikz@lib@place@handle@{#1}{corner north east}{0}{-1}{corner south east}{1}}

\tikzset{north left/.code =\tikz@lib@place@handle@{#1}{north east}{-1}{0}{north west}{1}}
\tikzset{north right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{0}{north east}{1}}
\tikzset{south left/.code =\tikz@lib@place@handle@{#1}{south east}{-1}{0}{south west}{1}}
\tikzset{south right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{0}{south east}{1}}

\tikzset{west above/.code =\tikz@lib@place@handle@{#1}{south west}{0}{1}{north west}{1}}
\tikzset{west below/.code=\tikz@lib@place@handle@{#1}{north west}{0}{-1}{south west}{1}}
\tikzset{east above/.code =\tikz@lib@place@handle@{#1}{south east}{0}{1}{north east}{1}}
\tikzset{east below/.code=\tikz@lib@place@handle@{#1}{north east}{0}{-1}{south east}{1}}

\newif\ifqrr@tikz@lib@place@postransform
\tikzset{node distance transformation/.is if=qrr@tikz@lib@place@postransform}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \ifqrr@tikz@lib@place@postransform
      \pgf@pos@transform{\pgf@x}{\pgf@y}% change from original
    \fi
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \pgfutil@in@{:}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@#1\tikz@stop
    \ifx\pgf@temp\pgfutil@empty
      \let\pgf@temp\tikz@node@distance
    \fi
    \pgfmathsetmacro\pgf@tempa{(\pgf@tempa)*#4}%
    \pgfmathsetmacro\pgf@tempb{(\pgf@tempb)*#3}%
    \edef\pgf@marshal{\noexpand\tikz@lib@place@handle@{\pgf@temp}{#2}{\pgf@tempb}{\pgf@tempa}{#5}{#6}}%
    \pgf@marshal
  \else
    \def\tikz@anchor{#2}%
    \let\tikz@do@auto@anchor=\relax%
    \edef\tikz@temp{#1}%
    \def\tikz@lib@place@single@factor{#6}%
    \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
  \fi
}
\def\tikz@lib@place@handle@qrr@#1:#2\tikz@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@@#1\tikz@stop
  \else
    \tikz@lib@place@handle@qrr@@#1and#1\tikz@stop
  \fi
  \def\pgf@temp{#2}%
}
\def\tikz@lib@place@handle@qrr@@#1and#2\tikz@stop{%
  \def\pgf@tempa{#1}%
  \def\pgf@tempb{#2}%
}
\def\qrr@xyshift@starred#1#2#3{
  \edef\tikz@marshal{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
  \tikz@marshal
  \ifpgfutil@in@
    \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
  \else
    \let#3\tikz@node@distance
  \fi
  \pgfmathparse{(#1)*#3}%
  \ifpgfmathunitsdeclared
    \if#2x%
      \pgftransformshift{\pgfqpoint{\pgfmathresult pt}{0pt}}%
    \else
      \pgftransformshift{\pgfqpoint{0pt}{\pgfmathresult pt}}%
    \fi
  \else
    \ifx#2x
      \pgf@process{\pgfqpointxy{\pgfmathresult}{0}}%
    \else
      \pgf@process{\pgfqpointxy{0}{\pgfmathresult}}%
    \fi
    \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi}
\tikzset{
  xshift*/.code=\qrr@xyshift@starred{#1}x\pgf@tempb,
  yshift*/.code=\qrr@xyshift@starred{#1}y\pgf@tempa,
}

\def\pgfutil@firstofmany#1#2\pgf@stop{#1}
\def\pgfutil@secondofmany#1#2\pgf@stop{#2}
\def\tikz@lib@place@of@#1#2#3{%
  \def\pgf@tempa{fit bounding box}%
  \edef\pgf@temp{\expandafter\pgfutil@firstofmany#2\pgf@stop}
  \if\pgf@temp(%
    \tikz@lib@place@fit@scan{#2}{0}%
  \else\if\pgf@temp|
      \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
    \else\ifx\pgf@temp\tikz@activebar
        \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
      \else\if\pgf@temp-
          \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{2}%
        \else\if\pgf@temp+
            \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{3}%
          \else
            \def\pgf@tempa{#2}%
          \fi
        \fi
      \fi
    \fi
  \fi
  \expandafter\tikz@scan@one@point\expandafter\tikz@lib@place@remember\expandafter(\pgf@tempa)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@fit@scan#1#2{
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  \if\pgfutil@firstofmany#1\pgf@stop(%
    \tikz@lib@fit@scan#1\pgf@stop%
  \else
    \tikz@lib@fit@scan(#1)\pgf@stop
  \fi
  \ifdim\pgf@xa>\pgf@xa
    % shouldn't happen
  \else
     \expandafter\def\csname pgf@sh@ns@fit bounding box\endcsname{rectangle}%
     \expandafter\edef\csname pgf@sh@np@fit bounding box\endcsname{%
       \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
       \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
     }%
     \expandafter\def\csname pgf@sh@nt@fit bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
     \expandafter\def\csname pgf@sh@pi@fit bounding box\endcsname{\pgfpictureid}%
     \ifcase#2\relax
     \or % 1 = vertical
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})}}}%
       \pgf@marshal
     \or % 2 = horizontal
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \or % 3 = both directions
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})},minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \fi
  \fi
}
\tikzset{
  fit bounding box/.code={\tikz@lib@place@fit@scan{#1}{0}},
  span vertical/.code={\tikz@lib@place@fit@scan{#1}{1}},
  span horizontal/.code={\tikz@lib@place@fit@scan{#1}{2}},
  span/.code={\tikz@lib@place@fit@scan{#1}{3}}}

\pgfmathdeclarefunction{x_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempb}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
\pgfmathdeclarefunction{y_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempa}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
%\tikzdeclarecoordinatesystem{node distance}{%
%  \tikz@cs@nd#1\tikz@stop}
%\def\tikz@cs@nd#1,#2\tikz@stop{%
%  \def\qrr@xyshift@starred@action##1{\pgftransformshift{##1}}%
%  \qrr@xyshift@starred{#1}x\pgf@tempb
%  \qrr@xyshift@starred{#2}y\pgf@tempa}
\endinput


==> tikzlibraryqrr.arc.code.tex <==
\tikzset{
  arc/ccw/.initial=1,
  arc/large/.initial=0,
  arc ccw/.style={/tikz/arc/ccw=1},
  arc cw/.style={/tikz/arc/ccw=0},
  arc large/.style={/tikz/arc/large=1},
  arc small/.style={/tikz/arc/large=0},
  arc rotation/.initial=0
}
\def\pgf@temp{2.10-cvs}
\ifx\pgfversion\pgf@temp\else
  \let\tikz@timer@arc\tikz@timer@line
\fi
\def\tikz@arcA rc{\pgfutil@ifnextchar t%
  {\tikz@flush@moveto\expandafter\expandafter\expandafter\tikz@arcB@cont\expandafter\pgfutil@gobble\pgfutil@gobble}
  {\tikz@flush@moveto\tikz@arc@cont}}
\def\tikz@arcB@cont{%
  \pgfutil@ifnextchar[\tikz@@do@arcB{
    \advance\tikz@expandcount by -10\relax% go down quickly
    \ifnum\tikz@expandcount<0\relax%
      \def\@next{\tikz@@do@arcB[]}%
    \else%
      \def\@next{\expandafter\tikz@arcB@cont}%
    \fi%
    \@next}}%
\def\tikz@@do@arcB[#1]{%
  \def\tikz@arcB@options{#1}%
  \tikz@do@@arcB}
\def\tikz@do@@arcB{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@do@@arcB}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@do@@arcB}
      {\tikz@scan@one@point\tikz@do@arcB}}}

\def\tikz@do@arcB#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \tikz@make@last@position{#1}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \iftikz@shapeborder
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \fi
  \begingroup
    \tikzset{every arc/.try}%
    \expandafter\tikzset\expandafter{\tikz@arcB@options}%
    \pgfmathparse{\pgfkeysvalueof{/tikz/x radius}}%
    \let\tikz@arc@x\pgfmathresult
    \ifpgfmathunitsdeclared
      \pgfmathparse{\pgfkeysvalueof{/tikz/y radius}}%
      \let\tikz@arc@y\pgfmathresult
      \ifpgfmathunitsdeclared
        \edef\tikz@arc@x{\tikz@arc@x pt}%
        \edef\tikz@arc@y{\tikz@arc@y pt}%
        \pgfpatharcto{\tikz@arc@x}{\tikz@arc@y}
                     {\pgfkeysvalueof{/tikz/arc rotation}}{\pgfkeysvalueof{/tikz/arc/large}}
                     {\pgfkeysvalueof{/tikz/arc/ccw}}{#1}%
      \else
        \tikzerror{You cannot mix dimensions and dimension values in an arc}%
      \fi
    \else
      \pgfmathparse{\pgfkeysvalueof{/tikz/y radius}}%
      \let\tikz@arc@y\pgfmathresult
      \ifpgfmathunitsdeclared
        \tikzerror{You cannot mix dimensions and dimension values in an arc}%
      \else
        \pgf@process{\pgfpointxy{\tikz@arc@x}{0}}%
        \pgfmathveclen@{\pgf@x}{\pgf@y}%
        \edef\tikz@arc@x{\pgfmathresult pt}%
        \pgf@process{\pgfpointxy{0}{\tikz@arc@y}}%
        \pgfmathveclen@{\pgf@x}{\pgf@y}%
        \edef\tikz@arc@y{\pgfmathresult pt}%
        \pgfpatharcto{\tikz@arc@x}{\tikz@arc@y}
                     {\pgfkeysvalueof{/tikz/arc rotation}}{\pgfkeysvalueof{/tikz/arc/large}}
                     {\pgfkeysvalueof{/tikz/arc/ccw}}{#1}%
      \fi
    \fi
  \endgroup
  \edef\tikz@timer@start@angle{\expandafter\expandafter\expandafter\pgfutil@firstoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \edef\tikz@timer@end@angle{\expandafter\expandafter\expandafter\pgfutil@secondoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\def
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikz@timer@zero@axis
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
  \expandafter\expandafter\expandafter\pgfutil@thirdoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\def
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikz@timer@ninety@axis
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
  \expandafter\expandafter\expandafter\pgfutil@fourthoffour\expandafter\pgfutil@gobble\pgf@marshal}%
  \let\tikz@timer=\tikz@timer@arc
  \tikz@scan@next@command
}
\def\pgfutil@firstoffour#1#2#3#4{#1}
\def\pgfutil@secondoffour#1#2#3#4{#2}
\def\pgfutil@thirdoffour#1#2#3#4{#3}
\def\pgfutil@fourthoffour#1#2#3#4{#4}


==> tikzlibraryqrr.misc.code.tex <==
%% full arc
\pgfset{full arc/.code=%
  \def\pgf@temp{#1}%
  \ifx\pgfutil@empty\pgf@temp
    \let\pgfmath@fullarc@factor\pgfutil@empty
  \else
    \pgfmathsetmacro\pgfmath@fullarc@factor{360/(#1)}%
  \fi,full arc=}
\pgfmathdeclareoperator{R}{full arc}{1}{postfix}{950}
\pgfmathdeclarefunction{full arc}{1}{%
  \begingroup
    \pgfmath@x=#1pt\relax
    \ifx\pgfmath@fullarc@factor\pgfutil@empty\else
      \pgfmath@x\pgfmath@fullarc@factor\pgfmath@x
    \fi
    \pgfmath@returnone\pgfmath@x
  \endgroup}

%% foreach
% http://tex.stackexchange.com/a/126418/16595
\def\pgffor@scanround(#1)#2,{\def\pgffor@value{(#1)#2}\pgffor@scanned}
% http://tex.stackexchange.com/a/126418/16595
\newif\ifqrr@pgf@foreach@no@list
\pgfqkeys{/pgf/foreach}{
  @use/.code args={#1to#2}{%
    \qrr@pgf@foreach@no@listtrue
    \qrr@pgf@foreach@no@list@use\foreachStart{#1}%
    \pgfutil@in@{step}{#2}
    \ifpgfutil@in@
      \qrr@pgf@foreach@no@list@parse@step#2\pgffor@stop
    \else
      \qrr@pgf@foreach@no@list@parse@step#2step1\pgffor@stop
    \fi
    \edef\qrr@pgf@foreach@no@list@list{\foreachStart,\foreachSecond,...,\foreachEnd}},
  use int/.code={%
    \let\qrr@pgf@foreach@no@list@use\pgfmathtruncatemacro
    \pgfkeysalso{/pgf/foreach/@use={#1}}},
  use float/.code={%
    \let\qrr@pgf@foreach@no@list@use\pgfmathsetmacro
    \pgfkeysalso{/pgf/foreach/@use={#1}}}}
\def\qrr@pgf@foreach@no@list@parse@step#1step#2\pgffor@stop{%
  \qrr@pgf@foreach@no@list@use\foreachEnd{#1}%
  \qrr@pgf@foreach@no@list@use\foreachSecond{\foreachStart+#2}}
\def\pgffor@vars{% manually extended, better etoolbox
  \pgfutil@ifnextchar i{\pgffor@@vars@end}{%
    \pgfutil@ifnextchar[{\pgffor@@vars@opt}{%]
      \pgfutil@ifnextchar/{\pgffor@@vars@slash@gobble}{%
         \ifqrr@pgf@foreach@no@list\expandafter\pgfutil@firstoftwo\else
           \expandafter\pgfutil@secondoftwo\fi
         {\qrr@pgf@foreach@no@listfalse\pgffor@macro@list\qrr@pgf@foreach@no@list@list}
         {\pgffor@@vars}}}}}%

%% Handlers
\pgfkeys{/handlers/.pgfmath/.code=\pgfmathparse{#1}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}
\pgfkeys{/handlers/.pgfmath int/.code=\pgfmathparse{int(#1)}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}
\pgfkeys{/handlers/.pgfmath strcat/.code=\pgfmathparse{strcat(#1)}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}

% http://tex.stackexchange.com/a/144187/16595
\pgfkeys{/handlers/.List/.code={%
    \let\pgfkeys@global@temp\pgfutil@empty
    \foreach \pgfkeys@temp in{#1}{
      \ifx\pgfkeys@global@temp\pgfutil@empty
        \global\let\pgfkeys@global@temp\pgfkeys@temp
      \else
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfkeys@global@temp\expandafter
          {\pgfkeys@temp}%
      \fi}%
    \expandafter\pgfkeys@exp@call\expandafter{\pgfkeys@global@temp}}}

%% PGFmath
\pgfmathdeclarefunction{strrepeat}{2}{%
  \begingroup\pgfmathint{#2}\pgfmath@count\pgfmathresult
    \let\pgfmathresult\pgfutil@empty
    \pgfutil@loop\ifnum\pgfmath@count>0\relax
      \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult#1}%
      \advance\pgfmath@count-1\relax
    \pgfutil@repeat\pgfmath@smuggleone\pgfmathresult\endgroup}

\pgfmathdeclarefunction{instr}{2}{%
  \pgfutil@in@{#1}{#2}%
  \ifpgfutil@in@\def\pgfmathresult{1}\else\def\pgfmathresult{0}\fi}

\pgfmathdeclarefunction{strcat}{...}{%
  \begingroup
    \let\pgfmathresult\pgfutil@empty
    \pgfmathstrcat@@#1\pgfmath@stop}
\def\pgfmathstrcat@@#1{%
  \ifx\pgfmath@stop#1%
    \let\pgfmath@next\pgfmathstrcat@@@
  \else
    \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult#1}%
    \let\pgfmath@next\pgfmathstrcat@@
  \fi
  \pgfmath@next}
\def\pgfmathstrcat@@@{\pgfmath@smuggleone\pgfmathresult\endgroup}


% the CVS version swaps the arguments so I define new atan
% functions that have the order of arguments in their name
\csname pgfmathatan2@\endcsname{0}{1}
\ifdim\pgfmathresult pt=0pt % atan2(y, x)
  \pgfmathdeclarefunction{atanXY}{2}{\csname pgfmathatan2@\endcsname{#2}{#1}}
  \pgfmathdeclarefunction{atanYX}{2}{\csname pgfmathatan2@\endcsname{#1}{#2}}
\else                       % atan2(x, y)
  \pgfmathdeclarefunction{atanXY}{2}{\csname pgfmathatan2@\endcsname{#1}{#2}}
  \pgfmathdeclarefunction{atanYX}{2}{\csname pgfmathatan2@\endcsname{#2}{#1}}
\fi

%% http://tex.stackexchange.com/a/141333/16595
\let\tikz@auto@anchor@orig      \tikz@auto@anchor
\let\tikz@auto@anchor@prime@orig\tikz@auto@anchor@prime
\tikzset{
  Auto/.code=\pgfkeysalso{/tikz/auto=#1}%
    \let\tikz@auto@anchor      \tikz@Auto@anchor
    \let\tikz@auto@anchor@prime\tikz@Auto@anchor@prime,
  auto/.prefix code=\let\tikz@auto@anchor      \tikz@auto@anchor@orig
                    \let\tikz@auto@anchor@prime\tikz@auto@anchor@prime@orig}
\def\tikz@Auto@anchor{%
  \pgfmathatanXY@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
  \pgfutil@tempdima=\pgfmathresult pt\relax
  \advance\pgfutil@tempdima-90pt\relax
  \edef\tikz@anchor{\pgf@sys@tonumber\pgfutil@tempdima}}
\def\tikz@Auto@anchor@prime{%
  \pgfmathatanXY@{\pgf@sys@tonumber\pgf@x}{\pgf@sys@tonumber\pgf@y}%
  \pgfutil@tempdima=\pgfmathresult pt\relax
  \advance\pgfutil@tempdima90pt\relax
  \edef\tikz@anchor{\pgf@sys@tonumber\pgfutil@tempdima}}

%% http://tex.stackexchange.com/a/132939/16595
\tikzset{
  @edges through/.code={{{% three braces to protect \pgfeov
    \pgfutil@ifnextchar[{\pgfkeysvalueof{/tikz/@@edges through/.@cmd}}
                        {\pgfkeysvalueof{/tikz/@@edges through/.@cmd}[]}#1\pgfeov}}},
  @@edges through/.style args={[#1]#2}{/tikz/insert path={edge[#1] (#2) (#2)}},
  edges through/.style={/tikz/@edges through/.list={#1}}}
\tikzset{
  @edges to/.code={{{% three braces to protect \pgfeov
    \pgfutil@ifnextchar[{\pgfkeysvalueof{/tikz/@@edges to/.@cmd}}
                        {\pgfkeysvalueof{/tikz/@@edges to/.@cmd}[]}#1\pgfeov}}},
  @@edges to/.style args={[#1]#2}{/tikz/insert path={edge[#1] (#2)}},
  edges to/.style={/tikz/@edges to/.list={#1}}}
\tikzset{
  @tos to/.code={{{% three braces to protect \pgfeov
    \pgfutil@ifnextchar[{\pgfkeysvalueof{/tikz/@@tos to/.@cmd}}
                        {\pgfkeysvalueof{/tikz/@@tos to/.@cmd}[]}#1\pgfeov}}},
  @@tos to/.style args={[#1]#2}{/tikz/insert path={to[#1] (#2)}},
  tos to/.style={/tikz/@tos to/.list={#1}}}


==> tikzlibraryqrr.shapes.openrectangle.code.tex <==
\usepgflibrary{qrr.shapes.openrectangle}
\endinput


==> tikzlibraryqrr.trans.code.tex <==
\usepgflibrary{qrr.trans}
\tikzset{
  mirror/.code={%
    \pgfutil@in@{--}{#1}%
    \ifpgfutil@in@
      \tikz@trans@mirror#1\@nil
    \else
      \tikz@scan@one@point\pgfqtransformmirror#1\relax
    \fi},
  ymirror/.code={\pgfutil@ifnextchar(\tikz@trans@ymirror@coordinate\tikz@trans@ymirror@simple#1\@nil},
  xmirror/.code={\pgfutil@ifnextchar(\tikz@trans@xmirror@coordinate\tikz@trans@xmirror@simple#1\@nil},
  mirror x/.code={%
    \pgfextract@process\tikz@temp{\tikz@scan@one@point\pgfutil@firstofone#1\relax}%
    \pgftransformmirror{\tikz@temp}{\pgfpointadd{\tikz@temp}{\pgfqpointxy{0}{1}}}},
  mirror y/.code={%
    \pgfextract@process\tikz@temp{\tikz@scan@one@point\pgfutil@firstofone#1\relax}%
    \pgftransformmirror{\tikz@temp}{\pgfpointadd{\tikz@temp}{\pgfqpointxy{1}{0}}}}
}
\def\tikz@trans@mirror#1--#2\@nil{%
  \pgftransformmirror{\tikz@scan@one@point\pgfutil@firstofone#1\relax}
                     {\tikz@scan@one@point\pgfutil@firstofone#2\relax}}
\def\tikz@trans@xmirror@simple#1\@nil{\pgftransformxmirror{#1}}
\def\tikz@trans@ymirror@simple#1\@nil{\pgftransformymirror{#1}}
\def\tikz@trans@xmirror@coordinate#1\@nil{%
  \tikz@scan@one@point\pgfutil@firstofone#1\pgftransformxmirror{+\the\pgf@x}}
\def\tikz@trans@ymirror@coordinate#1\@nil{\tikz@scan@one@point\pgfutil@firstofone#1\pgftransformymirror{+\the\pgf@y}}
\endinput


==> tikzlibraryshapes.qrr.roundedrectangle.code.tex <==
\usepgflibrary{intersections}%
\pgfset{
  rectangle with rounded corners north west radius/.initial=6pt,
  rectangle with rounded corners north east radius/.initial=6pt,
  rectangle with rounded corners south west radius/.initial=6pt,
  rectangle with rounded corners south east radius/.initial=6pt,
  rectangle with rounded corners radius/.style={
    /pgf/rectangle with rounded corners north west radius={#1},
    /pgf/rectangle with rounded corners north east radius={#1},
    /pgf/rectangle with rounded corners south west radius={#1},
    /pgf/rectangle with rounded corners south east radius={#1}}
}%
\newbox\pgfnodepartlowerbox
\pgfdeclareshape{split rectangle with rounded corners}{%
  \nodeparts{text,lower}%
  \savedmacro\splitrectanglewithroundedcornersparameter{%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/minimum height}}%
    %
    \pgf@xb\wd\pgfnodeparttextbox
    \advance\pgf@xb\ht\pgfnodeparttextbox
    \advance\pgf@xb\dp\pgfnodeparttextbox
    \pgf@yb\wd\pgfnodepartlowerbox
    \advance\pgf@yb\ht\pgfnodepartlowerbox
    \advance\pgf@yb\dp\pgfnodepartlowerbox
    \ifdim\pgf@yb>\pgf@xb
      \pgf@x\pgf@yb
    \else
      \pgf@x\pgf@xb
    \fi
    \pgf@y\pgf@x
    \advance\pgf@x2\pgf@xa
    \advance\pgf@y2\pgf@ya
    \ifdim\pgf@x<\pgf@xc
      \pgf@x\pgf@xc
    \fi
    \ifdim\pgf@y<\pgf@yc
      \pgf@y\pgf@yc
    \fi
    %
    \pgfutil@tempdima.5\pgf@x
    \pgfutil@tempdimb.5\pgf@y
    \edef\halfWidth{\the\pgfutil@tempdima}%
    \edef\halfHeight{\the\pgfutil@tempdimb}%
    \addtosavedmacro\halfWidth
    \addtosavedmacro\halfHeight
    %
    \advance\pgf@x-2\pgf@xa
    \advance\pgf@y-2\pgf@ya
%    \ifdim\pgf@x<\pgf@y
%      \pgf@x\pgf@y
%    \else
%      \pgf@y\pgf@x
%    \fi
    \pgfutil@tempdima\pgf@x
    \pgfutil@tempdimb\pgf@y
    \pgf@y-.5\pgf@y
    \advance\pgf@y\ht\pgfnodeparttextbox
    \pgf@x.5\pgf@x
    \pgfextract@process\centerpoint{}%
    \addtosavedmacro\centerpoint
    %
    \pgf@x\pgfutil@tempdima
    \pgf@y\pgfutil@tempdimb
    \advance\pgf@x-\wd\pgfnodepartlowerbox
    \advance\pgf@y-\ht\pgfnodeparttextbox
    \advance\pgf@y-\dp\pgfnodepartlowerbox
    \pgf@y-\pgf@y
    \pgfextract@process\loweranchor{}%
    \addtosavedmacro\loweranchor
    %
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/outer ysep}}%
    %
    \pgfextract@process\belownorthwest{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{-\halfWidth}{\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north west radius}}%
      \advance\pgf@y-\pgfutil@tempdima
      \advance\pgf@x-\pgf@xb
    }%
    \addtosavedmacro\belownorthwest
    %
    \pgfextract@process\leftnortheast{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{\halfWidth}{\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north east radius}}%
      \advance\pgf@x-\pgfutil@tempdima
      \advance\pgf@y\pgf@yb
    }%
    \addtosavedmacro\leftnortheast
    %
    \pgfextract@process\abovesoutheast{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{\halfWidth}{-\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south east radius}}%
      \advance\pgf@y\pgfutil@tempdima
      \advance\pgf@x\pgf@xb
    }%
    \addtosavedmacro\abovesoutheast
    %
    \pgfextract@process\rightsouthwest{%
      \pgfpointadd{\centerpoint}{\pgfqpoint{-\halfWidth}{-\halfHeight}}%
      \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south west radius}}%
      \advance\pgf@x\pgfutil@tempdima
      \advance\pgf@y-\pgf@yb
    }%
    \addtosavedmacro\rightsouthwest
  }%
  \anchor{lower}{\splitrectanglewithroundedcornersparameter\loweranchor}
  \anchor{center}{\splitrectanglewithroundedcornersparameter\centerpoint}
  \anchor{below north west}{\splitrectanglewithroundedcornersparameter\belownorthwest}
  \anchor{left north east}{\splitrectanglewithroundedcornersparameter\leftnortheast}
  \anchor{above south east}{\splitrectanglewithroundedcornersparameter\abovesoutheast}
  \anchor{right south west}{\splitrectanglewithroundedcornersparameter\rightsouthwest}
  \anchor{west}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@ya\pgf@y \belownorthwest\pgf@y\pgf@ya}
  \anchor{east}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@ya\pgf@y \abovesoutheast\pgf@y\pgf@ya}
  \anchor{north}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@xa\pgf@x \leftnortheast\pgf@x\pgf@xa}
  \anchor{south}{\splitrectanglewithroundedcornersparameter
    \centerpoint\pgf@xa\pgf@x \rightsouthwest\pgf@x\pgf@xa}
  \anchor{mid}{\splitrectanglewithroundedcornersparameter\centerpoint\pgfmathsetlength\pgf@y{+.5ex}}
  \anchor{mid west}{\splitrectanglewithroundedcornersparameter\belownorthwest\pgfmathsetlength\pgf@y{+.5ex}}
  \anchor{mid east}{\splitrectanglewithroundedcornersparameter\abovesoutheast\pgfmathsetlength\pgf@y{+.5ex}}
  \anchor{base}{\splitrectanglewithroundedcornersparameter\centerpoint\pgf@y0pt}
  \anchor{base west}{\splitrectanglewithroundedcornersparameter\belownorthwest\pgf@y0pt}
  \anchor{base east}{\splitrectanglewithroundedcornersparameter\abovesoutheast\pgf@y0pt}
  \anchor{north west}{\splitrectanglewithroundedcornersparameter
    \belownorthwest
    \pgf@xa\pgf@x
    \pgf@xb-\pgf@x
    \pgf@ya\pgf@y
    \leftnortheast
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \advance\pgf@xb\pgf@xa
    \pgfpointpolar{135}{\pgf@xb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{south west}{\splitrectanglewithroundedcornersparameter
    \rightsouthwest
    \pgf@xa\pgf@x
    \pgf@ya\pgf@y
    \pgf@yb-\pgf@y
    \belownorthwest
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \advance\pgf@yb\pgf@ya
    \pgfpointpolar{225}{\pgf@yb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{south east}{\splitrectanglewithroundedcornersparameter
    \abovesoutheast
    \pgf@ya\pgf@y
    \pgf@xb\pgf@x
    \pgf@xa\pgf@x
    \rightsouthwest
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \advance\pgf@xb-\pgf@xa
    \pgfpointpolar{315}{\pgf@xb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{north east}{\splitrectanglewithroundedcornersparameter
    \leftnortheast
    \pgf@xa\pgf@x
    \pgf@ya\pgf@y
    \pgf@yb\pgf@y
    \abovesoutheast
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \advance\pgf@yb-\pgf@ya
    \pgfpointpolar{45}{\pgf@yb}
    \advance\pgf@x\pgf@xa
    \advance\pgf@y\pgf@ya
  }
  \anchor{right north west}{\splitrectanglewithroundedcornersparameter
    \belownorthwest\pgf@xa\pgf@x\pgf@ya\pgf@y
    \leftnortheast\pgf@xb\pgf@x
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \pgf@x\pgf@xa
  }
  \anchor{below north east}{\splitrectanglewithroundedcornersparameter
    \leftnortheast\pgf@xa\pgf@x\pgf@ya\pgf@y
    \abovesoutheast\pgf@yb\pgf@y
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \pgf@y\pgf@ya
  }
  \anchor{left south east}{\splitrectanglewithroundedcornersparameter
    \abovesoutheast\pgf@xa\pgf@x\pgf@ya\pgf@y
    \rightsouthwest\pgf@xb\pgf@x
    \advance\pgf@xa\pgf@y
    \advance\pgf@xa-\pgf@ya
    \pgf@x\pgf@xa
  }%
  \anchor{above south west}{\splitrectanglewithroundedcornersparameter
    \rightsouthwest\pgf@xa\pgf@x\pgf@ya\pgf@y
    \belownorthwest\pgf@yb\pgf@y
    \advance\pgf@ya-\pgf@x
    \advance\pgf@ya\pgf@xa
    \pgf@y\pgf@ya
  }%
  \backgroundpath{%
    \splitrectanglewithroundedcornersparameter
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/outer ysep}}%
    \pgfpathmoveto{\pgfpointadd{\belownorthwest}{\pgfqpoint{\pgf@xb}{+0pt}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{above south west}}{\pgfqpoint{\pgf@xb}{+0pt}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south west radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\rightsouthwest}{\pgfqpoint{+0pt}{\pgf@yb}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{left south east}}{\pgfqpoint{+0pt}{\pgf@yb}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners south east radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\abovesoutheast}{\pgfqpoint{-\pgf@xb}{+0pt}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{below north east}}{\pgfqpoint{-\pgf@xb}{+0pt}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north east radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\leftnortheast}{\pgfqpoint{+0pt}{-\pgf@yb}}}%
    \pgfpathlineto{\pgfpointadd{\pgf@sh@reanchor{split rectangle with rounded corners}{right north west}}{\pgfqpoint{+0pt}{-\pgf@yb}}}%
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle with rounded corners north west radius}}%
    \pgfpatharcto{\pgfutil@tempdima}{\pgfutil@tempdima}{0}{0}{1}{\pgfpointadd{\belownorthwest}{\pgfqpoint{\pgf@xb}{+0pt}}}%
    \pgfpathclose
    \loweranchor
    \pgf@xa\pgf@x
    \advance\pgf@y-\dp\pgfnodepartlowerbox
    \pgfpathmoveto{\pgfqpoint{+0pt}{\pgf@y}}%
    \advance\pgf@xa\wd\pgfnodepartlowerbox
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\ht\pgfnodeparttextbox}}%
  }%
  \anchorborder{%
    \pgf@xb=\pgf@x
    \pgf@yb=\pgf@y
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{south}}%
    \pgf@ya\pgf@y
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{west}}%
    \pgf@xa\pgf@x
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{north}}%
    \pgf@yc\pgf@y
    \pgf@process{\pgf@sh@reanchor{split rectangle with rounded corners}{east}}%
    \pgf@y\pgf@yc
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@xa by\pgf@x%
    \advance\pgf@ya by\pgf@y%
    %
    \pgfutil@tempdima\pgf@xa
    \pgfutil@tempdimb\pgf@ya
%    \pgf@x\pgf@xa
%    \pgf@y\pgf@ya
    \splitrectanglewithroundedcornersparameter
    \centerpoint
    \pgf@xc\pgf@x
    \pgf@yc\pgf@y
    \ifdim\pgfutil@tempdima>\pgf@xc
      \ifdim\pgfutil@tempdimb>\pgf@yc % north east
        \pgf@lib@sh@qrr@get@radius@and@center0\pgfutil@tempdima\pgfutil@tempdimb
      \else                 % south east
        \pgf@lib@sh@qrr@get@radius@and@center3\pgfutil@tempdima\pgfutil@tempdimb
      \fi
    \else
      \ifdim\pgfutil@tempdimb>\pgf@yc % north west
        \pgf@lib@sh@qrr@get@radius@and@center1\pgfutil@tempdima\pgfutil@tempdimb
      \else                 % south west
        \pgf@lib@sh@qrr@get@radius@and@center2\pgfutil@tempdima\pgfutil@tempdimb
      \fi
    \fi
  }
}
\def\pgf@lib@sh@qrr@get@radius@and@center#1#2#3{%
  \begingroup
    \pgfutil@tempswafalse
    \ifcase#1% north east
      \def\pgf@tempa{1}%
      \leftnortheast
      \pgf@xa\pgf@x
      \pgf@ya\pgf@y
      \pgf@yb\pgf@y
      \abovesoutheast
      \advance\pgf@ya-\pgf@x
      \advance\pgf@ya\pgf@xa
      \advance\pgf@yb-\pgf@ya
      \ifdim#3>\pgf@ya
        \ifdim#2>\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \or      % north west
      \def\pgf@tempa{1}%
      \belownorthwest
      \pgf@xa\pgf@x
      \pgf@yb-\pgf@x
      \pgf@ya\pgf@y
      \leftnortheast
      \advance\pgf@xa\pgf@y
      \advance\pgf@xa-\pgf@ya
      \advance\pgf@yb\pgf@xa
      \ifdim#3>\pgf@ya
        \ifdim#2<\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \or      % south west
      \def\pgf@tempa{2}%
      \rightsouthwest
      \pgf@xa\pgf@x
      \pgf@ya\pgf@y
      \pgf@yb-\pgf@y
      \belownorthwest
      \advance\pgf@ya-\pgf@x
      \advance\pgf@ya\pgf@xa
      \advance\pgf@yb\pgf@ya
      \ifdim#3<\pgf@ya
        \ifdim#2<\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \else    % south east
      \def\pgf@tempa{2}%
      \abovesoutheast
      \pgf@ya\pgf@y
      \pgf@yb\pgf@x
      \pgf@xa\pgf@x
      \rightsouthwest
      \advance\pgf@xa\pgf@y
      \advance\pgf@xa-\pgf@ya
      \advance\pgf@yb-\pgf@xa
      \ifdim#3<\pgf@ya
        \ifdim#2>\pgf@xa
          \pgfutil@tempswatrue
        \fi
      \fi
    \fi
    \pgfinterruptboundingbox
      \ifpgfutil@tempswa
        \pgfintersectionofpaths{
          \pgfpathmoveto{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgfpathlineto{\pgfqpoint{#2}{#3}}%
        }{%
          \pgfpathcircle{\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgf@yb}%
        }%
        \pgfpointintersectionsolution{\pgf@tempa}
        \pgftransforminvert
        \pgfpointtransformed{}%
      \else
        \pgf@process{\pgfqpoint{#2}{#3}}%
      \fi
    \endpgfinterruptboundingbox
  \endgroup
}
\endinput

